Saying Hello World with Henshin - A Solution to the TTC 2011 Instructive Case

This paper gives an overview of the Henshin solution to the Hello World case study of the Transformation Tool Contest 2011, intended to show basic language concepts and constructs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{253}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.22}{10.4204/EPTCS.74.22}}
\pdfoutput=1

